Type Safe Extensible Programming

Software products evolve over time. Sometimes they evolve by adding new features, and sometimes by either fixing bugs or replacing outdated implementations with new ones. When software engineers fail to anticipate such evolution during development, they will eventually be forced to re-architect or re-build from scratch. Therefore, it has been common practice to prepare for changes so that software products are extensible over their lifetimes. However, making software extensible is challenging because it is difficult to anticipate successive changes and to provide adequate abstraction mechanisms over potential changes. Such extensibility mechanisms, furthermore, should not compromise any existing functionality during extension. Software engineers would benefit from a tool that provides a way to add extensions in a reliable way. It is natural to expect programming languages to serve this role. Extensible programming is one effort to address these issues. In this thesis, we present type safe extensible programming using the MLPolyR language. MLPolyR is an ML-like functional language whose type system provides type-safe extensibility mechanisms at several levels. After presenting the language, we will show how these extensibility mechanisms can be put to good use in the context of product line engineering. Product line engineering is an emerging software engineering paradigm that aims to manage variations, which originate from successive changes in software.

==> contents.tex <==
%
% Contents
%

\tableofcontents

\listoffigures

\listoftables


==> fig-il-sub.tex <==
%
% Substitution for IL
%

\begin{figure}
\[
\begin{array}{l}
n~[\vb/x] = n \qquad
x~[\vb/x] = \vb \qquad
y~[\vb/x] = y \mathbf{~if~} x \neq y \\[1mm]
(\eAbs{x:\taub}{\eb})~[\vb/x] = \eAbs{x:\taub}{\eb} \\[1mm] 
(\eAbs{y:\taub}{\eb})~[\vb/x] = \eAbs{y:\taub}{(\eb~[\vb/x])} 
                                \mathbf{~if~} x \neq y, y \notin \mathbf{FV}(\vb) \\[1mm]
(\eTabs{\alpha:\kappa}{\eb})~[\vb/x] = \eTabs{\alpha:\kappa}{(\eb~[\vb/x])} \\[1mm]
(\eb_1~\eb_2)~[\vb/x] = (\eb_1~[\vb/x])~(\eb_2~[\vb/x]) \qquad
(\eTapp{\eb}{\thetab})~[\vb/x] = \eTapp{(\eb~[\vb/x])}{\thetab} \\[1mm]
(\eLetrec{f:\taub}{\eAbs{x:\taub_2}{\eb_1}}{\eb_2})~[\vb/f] = 
				\eLetrec{f:\taub}{\eAbs{x:\taub_2}{\eb_1}}{\eb_2} \\[1mm]
(\eLetrec{f:\taub}{\eAbs{x:\taub_2}{\eb_1}}{\eb_2})~[\vb/x] = \\
~~~~~                  \eLetrec{f:\taub}{(\eAbs{x:\taub_2}{\eb_1})~[\vb/x]}{(\eb_2~[\vb/x])} 
                  \mathbf{~if~} x \neq f, f \notin \mathbf{FV}(\vb) \\[1mm]
(\eLetrec{f:\taub}{\eTabs{\alpha:\kappa}{\eb_1}}{\eb_2})~[\vb/f] = 
		  \eLetrec{f:\taub}{\eTabs{\alpha:\kappa}{\eb_1}}{\eb_2} \\[1mm] 
(\eLetrec{f:\taub}{\eTabs{\alpha:\kappa}{\eb_1}}{\eb_2})~[\vb/x] = \\
~~~~~                  \eLetrec{f:\taub}{\eTabs{\alpha:\kappa}{(\eb_1~[\vb/x])}}{(\eb_2~[\vb/x])}
                  \mathbf{~if~} x \neq f, f \notin \mathbf{FV}(\vb) \\[1mm]
(\eLet{x:\taub}{\eb_1}{\eb_2})~[\vb/x] = \eLet{x:\taub}{(\eb_1~[\vb/x])}{\eb_2} \\[1mm]
(\eLet{y:\taub}{\eb_1}{\eb_2})~[\vb/x] = \\
~~~~~                  \eLet{x:\taub}{(\eb_1~[\vb/x]}{(\eb_2~[\vb/x])} 
                  \mathbf{~if~} x \neq f, y \notin \mathbf{FV}(\vb) \\[1mm]
(\eRecN{i=1}{n}{l_i = \eb_i})~[\vb/x] = \eRecN{i=1}{n}{l_i = \eb_i~[\vb/x]} \\[1mm]
(\eRecExt{\eb_1}{\eRec{l=\eb_2}})~[\vb/x] = 
                  \eRecExt{(\eb_1~[\vb/x])}{\eRec{l=\eb_2~[\vb/x]}} \\[1mm]
(\eRecSub{\eb}{l})~[\vb/x] = \eRecSub{(\eb~[\vb/x])}{l} \qquad
(\eb.l)~[\vb/x] = (\eb~[\vb/x]).l \\[2mm]
(\reify{\rhob}{\taub}{\eb})~[\vb/x] = \reify{\rhob}{\taub}{(\eb~[\vb/x])}
\end{array}
\]
\caption{Substituting $\vb$ for free variable $x$, $\eb~[\vb/x]$}
\label{fig:il-subs-1}
\end{figure}

\begin{figure}
\[
\begin{array}{l}
n~[\thetab/\alpha] = n \qquad
x~[\thetab/\alpha] = x \\[1mm]
(\eAbs{x:\taub'}{\eb})~[\thetab/\alpha] = 
                  \eAbs{x:\taub'~[\thetab/\alpha]}{(\eb~[\thetab/\alpha])} \\[1mm] 
(\eTabs{\alpha:\kappa}{\eb})~[\thetab/\alpha] = \eTabs{\alpha:\kappa}{\eb} \\[1mm]
(\eTabs{\beta:\kappa}{\eb})~[\thetab/\alpha] = 
                  \eTabs{\beta:\kappa}{(\eb~[\thetab/\alpha])}
                  \mathbf{~if~} \alpha \neq \beta, \beta \notin \mathbf{FTV}(\thetab) \\[1mm]
(\eb_1~\eb_2)~[\thetab/\alpha] = (\eb_1~[\thetab/\alpha])~(\eb_2~[\thetab/\alpha]) \qquad
(\eTapp{\eb}{\thetab'})~[\thetab/\alpha] = \eTapp{(\eb~[\thetab/\alpha])}{\thetab'} \\[1mm]
(\eLetrec{f:\taub_1}{\eAbs{x:\taub_2}{\eb_1}}{\eb_2})~[\thetab/\alpha] = \\
~~~~~             \eLetrec{f:\taub_1~[\thetab/\alpha]}
                  {\eAbs{x:\taub_2~[\thetab/\alpha]}{(\eb_1~[\thetab/\alpha])}}
                  {(\eb_2~[\thetab/\alpha])} \\[1mm]
(\eLetrec{f:\taub'}{\eTabs{\alpha:\kappa}{\eb_1}}{\eb_2})~[\thetab/\alpha] = \\
~~~~~             \eLetrec{f:\taub'~[\thetab/\alpha]}
                  {\eTabs{\alpha:\kappa}{\eb_1}}{(\eb_2~[\thetab/\alpha])} \\[1mm] 
(\eLetrec{f:\taub'}{\eTabs{\beta:\kappa}{\eb_1}}{\eb_2})~[\thetab/\alpha] = \\
~~~~~            \eLetrec{f:\taub~[\thetab/\alpha]}
                 {\eTabs{\beta:\kappa}{(\eb_1~[\thetab/\alpha])}}{(\eb_2~[\thetab/\alpha])}
\mathbf{~if~} \alpha \neq \beta, \beta \notin \mathbf{FTV}(\thetab) \\[1mm]
(\eLet{x:\taub'}{\eb_1}{\eb_2})~[\thetab/\alpha] = 
           \eLet{x:\taub'~[\thetab/\alpha]}
                {(\eb_1~[\thetab/\alpha])}{(\eb_2~[\thetab/\alpha])} \\[1mm]
(\eRecN{i=1}{n}{l_i = \eb_i})~[\thetab/\alpha] = 
                \eRecN{i=1}{n}{l_i = \eb_i~[\thetab/\alpha]} \\[1mm]
(\eRecExt{\eb_1}{\eRec{l=\eb_2}})~[\thetab/\alpha] = 
                  \eRecExt{(\eb_1~[\thetab/\alpha])}{\eRec{l=\eb_2~[\thetab/\alpha]}} \\[1mm]
(\eRecSub{\eb}{l})~[\thetab/\alpha] = \eRecSub{(\eb~[\thetab/\alpha])}{l} \qquad
(\eb.l)~[\thetab/\alpha] = (\eb~[\thetab/\alpha]).l \\[2mm]
(\reify{\rhob}{\taub'}{\eb})~[\thetab/\alpha] = 
                  \reify{\rhob~[\thetab/\alpha]}{\taub~[\thetab/\alpha]}{(\eb~[\thetab/\alpha])}
\end{array}
\]
\caption{Substituting $\thetab$ for free type variable $\alpha$, $\eb~[\thetab/\alpha]$}
\label{fig:il-subs-2}
\end{figure}

\begin{figure}
\[
\begin{array}{l}
\alpha~[\thetab/\alpha] = \thetab \qquad
\beta~[\thetab/\alpha] = \beta \mathbf{~if~} \alpha \neq \beta \qquad
\Int~[\thetab/\alpha] = \Int \\[1mm]
(\taub_1 \ra \taub_2)~[\thetab/\alpha] = 
             (\taub_1~[\thetab/\alpha]) \ra (\taub_2~[\thetab/\alpha]) \\[1mm]
(\forall\alpha:\kappa.\taub)~[\thetab/\alpha] =
             \forall\alpha:\kappa.\taub \\[1mm]
(\forall\beta:\kappa.\taub)~[\thetab/\alpha] =
             \forall\beta:\kappa.(\taub~[\thetab/\alpha]) 
             \mathbf{~if~} \alpha \neq \beta, \beta \notin \mathbf{FTV}(\theta) \\[1mm]
\tRec{\rhob}~[\thetab/\alpha] = \tRec{\rhob~[\thetab/\alpha]} \qquad
\tRowEmp~[\thetab/\alpha] = \tRowEmp \\[1mm]
(l:\taub, \rhob)~[\thetab/\alpha] = l:\taub'~[\thetab/\alpha], \rhob~[\thetab/\alpha] \\[1mm]
(\alpha \rowArrow \taub)~[\thetab/\alpha] = \thetab \rowArrow (\taub'~[\thetab/\alpha]) \\[1mm]
(\beta \rowArrow \taub)~[\thetab/\alpha] = 
             \beta \rowArrow (\taub'~[\thetab/\alpha]) 
             \mathbf{~if~} \alpha \neq \beta
\end{array}
\]

\caption{Substituting $\thetab$ for free type variable $\alpha$, $\thetab'~[\thetab/\alpha]$}
\label{fig:il-subs-3}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-lrec-eval.tex <==
\begin{figure}[t]
\begin{mathpar}
\irr{\rlabel{val}}
{ }
{v \Downarrow v}{}
%
\and
%
\irr{\rlabel{plus}}
{
t_1 \Downarrow n_1 \+
t_2 \Downarrow n_2
}
{t_1 + t_2 \Downarrow n_1 + n_2}
%
\and
%
\irr{\rlabel{minus}}
{
t_1 \Downarrow n_1 \+
t_2 \Downarrow n_2
}
{t_1 - t_2 \Downarrow n_1 - n_2}
%
\and
%
\irr{\rlabel{app}}
{
t_1 \Downarrow \eFun{f}{x}{t_1'} \+
t_2 \Downarrow v_2 \+
t_1' [\eFun{f}{x}{t_1'}/f_1, v_2/x] \Downarrow v
}
{t_1~t_2 \Downarrow v}
%
\and
%
\irr{\rlabel{let}}
{
t_1 \Downarrow v_1 \+
t_2 [v_1/x] \Downarrow v
}
{\eLet{x}{t_1}{t_2} \Downarrow v}
%
\and
%
\irr{\rlabel{length}}
{t \Downarrow \elRec{v_0,\ldots,v_{n-1}}}
{\eLength{t} \Downarrow n}
%
\and
%
\irr{\rlabel{select}}
{
t_1 \Downarrow \elRec{v_0, \ldots, v_i, \ldots, v_{n-1}} \+
t_2 \Downarrow i \+
0 \leq i < n
}
{t_1.t_2 \Downarrow v_i}
%
\and
%
\irr{\rlabel{tuple}}
{
s_1 \Downarrow_s {v_{1,0}, \ldots, v_{1,k_1-1}} \+ \ldots \+
s_n \Downarrow_s {v_{n,0}, \ldots, v_{n,k_n-1}}
}
{
\elRec{s_1, \ldots, s_n} \Downarrow
\elRec{v_{1,0}, \ldots, v_{1,k_1-1}, \ldots, v_{n,0}, \ldots, v_{n,k_n-1}}
}
%
\and
%
\irr{\rlabel{slice/singleton}}
{t \Downarrow v}
{t \Downarrow_s v}
%
\and
%
\irr{\rlabel{slice/sequence}}
{
t_1 \Downarrow \elRec{v_0, \ldots, v_i, \ldots, v_j, \ldots, v_{n-1}} \+
t_2 \Downarrow i \+
t_3 \Downarrow j \+
0 \leq i \leq j \leq n
}
{(t_1, t_2, t_3) \Downarrow_s v_i, \ldots, v_{j-1}}
\end{mathpar}
\caption{The dynamic semantics for \lambdarec.}
\label{fig:lambda::dynamic-semantics}
\end{figure}


==> fig-lrec-static.tex <==
\begin{figure}[t]
\[
\begin{array}{lrrl}
%% Value & Type
\mathsf{Types} &
\tauu & \bnfdef & \Int \bnfalt \tauu_1 \ra \tauu_2 \bnfalt
                  \elRecN{i=0}{n-1}{\tauu_i} \bnfalt \idx{l}{\tauu} \\
%% Typing environment
\mathsf{Typenv} &
\Gammau & \bnfdef & \varnothing \bnfalt \Gammau, x \mapsto \tauu \\

%% Index judgement
\mathsf{Index} &
\Lu & \bnfdef & \varnothing \bnfalt \Lu, I \mapsto \idx{l}{\tauu} \\[2mm]
\end{array}
\]

\begin{mathpar}
\irr{\rlabel{val}}
{ }
{\Gammau \ts n : \Int }
%
\and
%
\irr{\rlabel{plus}}
{
\Gammau \ts t_1 : \Int \+
\Gammau \ts t_2 : \Int
}
{\Gammau \ts t_1 + t_2 : \Int }
%
\and
%
\irr{\rlabel{minus}}
{
\Gammau \ts t_1 : \Int \+
\Gammau \ts t_2 : \Int
}
{\Gammau \ts t_1 - t_2 : \Int }
%
\and
%
\irr{\rlabel{fun}}
{
\Gammau,x:\tauu' \ts t : \tauu \+
}
{\Gammau \ts \eAbs{x}{t} : \tauu' \ra \tauu}
%
\and
%
\irr{\rlabel{app}}
{
\Gammau \ts t_1 : \tauu_2 \ra \tauu \+
\Gammau \ts t_2 : \tauu_2 
}
{\Gammau \ts t_1~t_2 : \tauu}
%
\and
%
\irr{\rlabel{let}}
{
\Gammau \ts t_1 : \tauu_1 \+
\Gammau,x:\tauu_1 \ts t_2 : \tauu
}
{\Gammau \ts \eLet{x}{t_1}{t_2} : \tauu}
%
\and
%
\irr{\rlabel{letrec}}
{
\Gammau \ts t_1 : \tauu_1 \+
\Gammau,f:\tauu' \ra \tauu_1,x:\tauu' \ts t_2 : \tauu
}
{\Gammau \ts \eLetrec{f}{\eAbs{x}{t_1}}{t_2} : \tauu}
%
\and
%
\irr{\rlabel{length}}
{\Gammau \ts t : \elRecN{i=0}{n-1}{l_i:\tauu_i}}
{\Gammau \ts \eLength{t} : \Int}
%
\and
%
\irr{\rlabel{select}}
{
\Gammau \ts t : \tauu \+
\tauu = \elRec{l_0:\tauu_0, \ldots, l_i:\tauu_i, \ldots, l_{n-1}:\tauu_{n-1}} \+
\Lu \ts I : \idx{l_i}{\tauu} \+
0 \leq i < n
}
{\Lu;\Gammau \ts t.I : \tauu_i}
%
\and
%
\irr{\rlabel{tuple}}
{
\Gammau \ts_s s_1 : {l_{1,0}:\tauu_{1,0}, \ldots, 
                     l_{1,k_1-1}:\tauu_{1,k_1-1}} \+\+ 
\ldots \+\+
\Gammau \ts_s s_n : {l_{n,0}:\tauu_{n,0}, \ldots, 
                     l_{n,k_n-1}:\tauu_{n,k_n-1}}
}
{
\Gammau \ts \elRec{s_1, \ldots, s_n} :
            \elRec{l_{1,0}:\tauu_{1,0}, \ldots, 
                   l_{1,k_1-1}:\tauu_{1,k_1-1}, \ldots, 
                   l_{n,0}:\tauu_{n,0}, \ldots, 
                   l_{n,k_n-1}:\tauu_{n,k_n-1}}
}
%
\and
%
\irr{\rlabel{slice/singleton}}
{\Gammau \ts t : l:\tauu}
{\Gammau \ts_s t : l:\tauu}
%
\and
%
\irr{\rlabel{slice/sequence}}
{
\Gammau \ts t_1 : \tauu_1 \+
\tauu_1 = \elRec{l_0:\tauu_0, \ldots, 
                         l_i:\tauu_i, \ldots, 
                         l_j:\tauu_j, \ldots, 
                         l_{n-1}:\tauu_{n-1}} \+
\Lu \ts I_2 : \idx{l_i}{\tauu_1} \+
\Lu \ts I_3 : \idx{l_j}{\tauu_1} \+
0 \leq i \leq \j \leq n
}
{\Lu;\Gammau \ts_s (t_1, I_2, I_3) : l_i:\tauu_i, \ldots, l_{j-1}:\tauu_{j-1}}
%
\and
%
\irr{\rlabel{ifun}}
{
\Lu,I:\idx{l}{\tauu'};\Gammau \ts t : \tauu \+
}
{\Lu;\Gammau \ts \eAbs{I}{t} : \idx{l}{\tauu'} \ra \tauu}
%
\and
%
\irr{\rlabel{iapp}}
{
\Gammau \ts t : \idx{l}{\tauu'} \ra \tauu \+
\Lu \ts I : \idx{l}{\tauu'}
}
{\Lu;\Gammau \ts t~I : \tauu}
\end{mathpar}
\caption{The typing rules for \lambdarec.}
\label{fig:lambda::static-semantics}
\end{figure}


==> fig-lrec-trans.tex <==
\begin{figure}
\begin{mathpar}
\irr{\rlabel{int}}
{ }
{\Sigma \ts n \vartriangleright n}
%
\and
%
\irr{\rlabel{var}}
{ }
{\Sigma \ts x \fmaps x}
{\strut}
%
\and
%
\irr{\rlabel{fun}}
{\Sigma \ts \eb \fmaps t}
{\Sigma \ts \eAbs{x:\taub}{\eb} \fmaps \eFun{f}{x}{t}}
%
\and
%
\irr{\rlabel{app}}
{\Sigma \ts \eb_1 \fmaps t_1 \+ \Sigma \ts \eb_2 \fmaps t_2}
{\Sigma \ts \eb_1~\eb_2 \fmaps t_1~t_2}
%
\and
%
\irr{\rlabel{let}}
{\Sigma \ts \eb_1 \fmaps t_1 \+  \Sigma \ts \eb_2 \fmaps t_2}
{\Sigma \ts \eLet{x:\taub}{\eb_1}{\eb_2} \fmaps \eLet{x}{t_1}{t_2}}
%
\and
%
\irr{\rlabel{select}}
{
\Sigma \ts \eb \fmaps t \+ t' = \indexOf{\Sigma}{l}{\labelsOf{\typeOf{\eb}}}
}
{\Sigma \ts \eb.l \fmaps t.t'}
%
\and
%
\irr{\rlabel{r}}
{
\forall i,j. i<j \Rightarrow l_{\#(i)} <_l l_{\#(j)} \+
\{l_{\#(1)}, \ldots, l_{\#(n)} \} = \{l_1, \ldots, l_n\} \+
\forall i. \left( \Sigma \ts \eb_i \fmaps t_i \right)
}
{
\Sigma  \ts      \eRecN{i=1}{n}{l_i = \eb_i}
\fmaps \eLet{x_1}{t_1}{\ldots\eLet{x_n}{t_n}{\elRecN{i=1}{n}{x_{\#(i)}}}}
}
%
\and
%
\irr{\rlabel{r/ext}}
{
\Sigma \ts \eb_1 \fmaps t_1 \qquad \Sigma \ts \eb_2 \fmaps t_2 \+
t_0 = \indexOf{\Sigma}{l}{\labelsOf{\typeOf{\eb_1}}}
%x_1 \mbox{~fresh} \\
%s_1 = (x_1, 0, t_0) \qquad
%s_2 = (x_1, t_0, \eLength{x_1})
}
{
\Sigma  \ts     \eRecExt{\eb_1}{\eRec{l=\eb_2}} 
        \fmaps \eLet{x}{t_1}{\elRec{(x, 0, t_0) ,t_2,(x, t_0, \eLength{x})}}
}
%
\and
%
\irr{\rlabel{r/sub}}
{
\Sigma \ts \eb \fmaps t \+
t_0 = \indexOf{\Sigma}{l}{\labelsOf{\typeOf{\eb}}}
%s_1 = (x, 0, t_0) \qquad s_2 = (x, t_0+1, \eLength{x})\\
}
{
\Sigma  \ts     \eRecSub{\eb}{l} 
        \fmaps  \eLet{x}{t}{\elRec{(x, 0, t_0), (x, t_0+1, \eLength{x})}}
}
%
\and
%
\irr{\rlabel{ty/abs}}
{
%\Sigma,\ldots,\beta_i\hasKind\{(l_i^1, x_i^1),\ldots,(l_i^{m_i},x_i^{m_i})\},\ldots
%\ts \eb  \fmaps t \+
%\forall i.~ 1 \le i \le n.~\kappa_i = \{ l_i^1, \ldots, l_i^{m_i} \}
\Sigma,\alpha:\{(l_1,x_1), \ldots, (l_n,x_n)\} \ts \eb \fmaps t \+
\kappa = \{ l_1, \ldots, l_n \}
}
{
%\Sigma  \ts  \Lambda (\alpha_1, \alpha_k).\Lambda~(\beta_1 \hasKind \kappa_1, \ldots, \beta_n \hasKind \kappa_n). \eb 
% \fmaps  \lambda x_1^1 \ldots \lambda x_1^{m_1} \ldots \lambda x_n^1 \ldots \lambda x_n^{m_n}.~t
\Sigma  \ts  \Lambda \alpha:\kappa.\eb \fmaps  
\lambda x_1 \ldots \lambda x_n.~t
}
%
\and
%
\irr{\rlabel{ty/app}}
{
%\Sigma \ts \eb \fmaps t \+
%\typeOf{e}  =  \forall~(\beta_1 \hasKind \kappa_1 \ldots \beta_n \hasKind \kappa_n).~\taub \+
%\forall i.~ 1 \le i \le n.~\kappa_i  =   \{ l_i^1, \ldots, l_i^{m_i} \} \+
%\forall i \in \{1,\ldots,n\} \forall j \in \{1,\ldots,m_i\} . 
%t_i^j =  \indexOf{\Sigma}{l_i^j}{(L_i \cup \kappa_i, \rho'_i)} \+ 
%\mbox{where~} (L_i,\rho'_i) = \labelsOf{\{\rhob_i\}}
\Sigma \ts \eb \fmaps t \+
\typeOf{e}  =  \forall~\alpha:\kappa.\taub \+
\kappa  =   \{ l_i, \ldots, l_n \} \+
\forall i \in \{1,\ldots,n\} . 
t_i =  \indexOf{\Sigma}{l_i}{(L, \rhob)} \+ 
\mbox{where~} (L,\rhob) = \labelsOf{\thetab}
}
{
\Sigma
 \ts     \eb[\thetab]
 \fmaps  t~t_1 \ldots t_n
}
\end{mathpar}
\caption{The translation from the \IL{} into the \lambdarec language.}
\label{fig:lambda::systemf-lambda}
\end{figure}


==> fig-mod-trans.tex <==
%
% Translation from the module into the core
%

\begin{figure}
\begin{mathpar}
\irr{(Introduction)}
{
}
{
\begin{array}{crcl}
         & \mathsf{module}~X & = & \{\{\eVal{v_1}{e_1},\ldots,\eVal{v_n}{e_n}\}\} \\
\leadsto & \mathsf{val}~X   & = & \mathsf{let} ~~ \eVal{v_1}{e_1} \\
         &                   &   & ~~~~~ \ldots \\
         &                   &   & ~~~~~ \eVal{v_n}{e_n} \\
         &                   &   & \mathsf{in~~} \eRec{v_1' = v_1,\ldots,v_n'=v_n}\\
         &                   &   & \mathsf{end} \\[4mm]
\end{array}
}
%
\and
%
\irr{(Template)}
{
}
{
\begin{array}{crclll}
         & \mathsf{template}~X & & (X_1,\ldots,X_i,\ldots,X_n)
                                 & = & \{\{\ldots,\eVal{v_i}{X_i.l},\ldots\}\} \\
\leadsto & \mathsf{val}~X & = & \mathsf{fn} ~~~ (X_1,\ldots,X_n) & => & 
                                  \mathsf{let}~\eVal{v_1}{e_1}\\
&&&         &                   & ~~~~~ \ldots \\
&&&         &                   & ~~~~~ \eVal{v_i}{X_i.l}\\
&&&         &                   & ~~~~~ \ldots \\
&&&         &                   & ~~~~~ \eVal{v_n}{e_n} \\
&&&         &                   & \mathsf{in} ~~~ \eRec{v_1' = v_1,\ldots,v_n'=v_n}\\
&&&	 &	             & \mathsf{end} \\[4mm]
\end{array}
}
%
\and
%
\irr{(Extension)}
{
\eMod{\_}{M} ~~ \leadsto ~~ r
}
{
\begin{array}{crcl}
         & \mathsf{module}~X~ & = & M~\boxplus~\{\{\eVal{v}{e}\}\} \\
\leadsto & \mathsf{val}~X    & = & \mathsf{let} ~~ \eVal{v}{e} \\
         &                    &   & \mathsf{in}  ~~ r\otimes\eRec{v' = v}\\
         &                    &   & \mathsf{end} \\
\end{array} 
}
%
\and
%
\irr{(Subtraction)}
{
\eMod{\_}{M} ~~ \leadsto ~~ r
}
{
\begin{array}{crcl}
         & \mathsf{module}~X & = & M~\boxminus~l \\
\leadsto & \mathsf{val}~~X   & = & r\oslash l \\[4mm]
\end{array}
}
%
\and
%
\irr{(Application)}
{
\forall i.M_i \leadsto r_i \+
T \leadsto r
}
{
\begin{array}{crcl}
         & \mathsf{module}~X & = & T~(M_1,\ldots,M_n) \\
\leadsto & \mathsf{val}~~X   & = & r~(r_1,\ldots,r_n) \\
\end{array}
}
\end{mathpar}
\caption{The translation from the module language into the core
language.}
\label{fig:trans-module}
\end{figure}



==> lrec-prop.tex <==
\subsection{Properties of \lambdarec}

\begin{lemma}[Correctness of translation~$\leadsto$]
If $\Delta;\Gamma \ts e:\tau;\rho \leadsto \cb :\comp{\taub}{\rhob}$ and $\Gammab \supseteq C(\Gamma)$
and $\Deltab \supseteq C(\Delta)$,
then $\Deltab;\Gammab \ts \cb : \comp{\taub}{\rhob}$.
\end{lemma}

\begin{proof}
By induction of a derivation of $\Delta;\Gamma \ts e:\tau;\rho \leadsto \cb :\comp{\taub}{\rhob}$.
\end{proof}

